Your Text Encoder Can Be An Object-Level Watermarking Controller

Invisible watermarking of AI-generated images can help with copyright protection, enabling detection and identification of AI-generated media. In this work, we present a novel approach to watermark images of T2I Latent Diffusion Models (LDMs). By only fine-tuning text token embeddings $W_*$, we enable watermarking in selected objects or parts of the image, offering greater flexibility compared to traditional full-image watermarking. Our method leverages the text encoder's compatibility across various LDMs, allowing plug-and-play integration for different LDMs. Moreover, introducing the watermark early in the encoding stage improves robustness to adversarial perturbations in later stages of the pipeline. Our approach achieves $99\%$ bit accuracy ($48$ bits) with a $10^5 \times$ reduction in model parameters, enabling efficient watermarking.

==> sec/algos/algo-1_object_level_watermarking.tex <==
\begin{algorithm}[!ht]
    \begin{minipage}{\linewidth}
        \caption{Inference: Object-Level Watermarking}\label{alg:object_level_watermarking}
        \begin{algorithmic}[1]
            \Require \textbf{Input} Object to watermark $O^{i}$, Text-to-image prompt $\mathcal{P}$, Diffusion pipeline $\mathcal{D}$, Watermarking token $\mathcal{W}$
            
            \State $\mathcal{D} \gets \mathcal{D} \cup \mathcal{W}$
            \State $\mathbf{x}_T \sim \mathcal{N}(0, I)$
            
            \For{$T = 50, \dots, \tau^*$}
                \State \hspace{1em} $\mathbf{z} \sim \mathcal{N}(0, I)$ if $t > 1$, else $\mathbf{z} = 0$
                \State \hspace{1em} $\mathbf{x}_{t-1} = \frac{1}{\sqrt{\alpha_t}} \left( \mathbf{x}_t - \frac{1 - \alpha_t}{\sqrt{1 - \bar{\alpha}_t}} \epsilon_\theta(\mathbf{x}_t, \mathcal{P}, t) \right) + \sigma_t \mathbf{z}$
            \EndFor
            \vspace{0.5em}

            \For{$t = \tau^*, \dots, 0$}
                \State \hspace{1em} $\mathcal{P} \gets \mathcal{P} + \mathcal{W}$
                \State \hspace{1em} $\mathcal{A}_{O^i}^{(t)} \gets (1 - \lambda) \cdot \mathcal{A}_{O^i}^{(t)} + \lambda \cdot \mathcal{A}_{\mathcal{W}}^{(t)}$
                \State \hspace{1em} $\mathbf{x}_{t-1} = \frac{1}{\sqrt{\alpha_t}} \left( \mathbf{x}_t - \frac{1 - \alpha_t}{\sqrt{1 - \bar{\alpha}_t}} \epsilon_\theta(\mathbf{x}_t, \mathcal{P}, t) \right) + \sigma_t \mathbf{z}$
            \EndFor
            \vspace{0.5em}
            
            \State \Return $\text{watermarked\_image}$
        \end{algorithmic} 
    \end{minipage}
\end{algorithm}



\vspace*{-10pt}

==> sec/algos/suppl_heatmap_algo.tex <==
\begin{algorithm}[!ht]
    \begin{minipage}{\linewidth}
        \caption{Inference: Object-Level Watermarking}\label{alg:object_level_watermarking}
        \begin{algorithmic}[1]
            \Require \textbf{Input} Object to watermark $O^{i}$, Text-to-image prompt $\mathcal{P}$, Diffusion pipeline $\mathcal{D}$, Watermarking token $\mathcal{W}$
            
            \State $\mathcal{D} \gets \mathcal{D} \cup \mathcal{W}$
            \State $\mathbf{x}_T \sim \mathcal{N}(0, I)$
            
            \For{$T = 50, \dots, \tau^*$}
                \State \hspace{1em} $\mathbf{z} \sim \mathcal{N}(0, I)$ if $t > 1$, else $\mathbf{z} = 0$
                \State \hspace{1em} $\mathbf{x}_{t-1} = \frac{1}{\sqrt{\alpha_t}} \left( \mathbf{x}_t - \frac{1 - \alpha_t}{\sqrt{1 - \bar{\alpha}_t}} \epsilon_\theta(\mathbf{x}_t, \mathcal{P}, t) \right) + \sigma_t \mathbf{z}$
            \EndFor
            \vspace{0.5em}

            \For{$t = \tau^*, \dots, 0$}
                \State \hspace{1em} $\mathcal{P} \gets \mathcal{P} + \mathcal{W}$
                \State \hspace{1em} $\mathcal{A}_{O^i}^{(t)} \gets (1 - \lambda) \cdot \mathcal{A}_{O^i}^{(t)} + \lambda \cdot \mathcal{A}_{\mathcal{W}}^{(t)}$
                \State \hspace{1em} $\mathbf{x}_{t-1} = \frac{1}{\sqrt{\alpha_t}} \left( \mathbf{x}_t - \frac{1 - \alpha_t}{\sqrt{1 - \bar{\alpha}_t}} \epsilon_\theta(\mathbf{x}_t, \mathcal{P}, t) \right) + \sigma_t \mathbf{z}$
            \EndFor
            \vspace{0.5em}
            
            \State \Return $\text{watermarked\_image}$
        \end{algorithmic} 
    \end{minipage}
\end{algorithm}



\vspace*{-10pt}

==> sec/archive.tex <==
\begin{figure}[H]
\centering
    \scriptsize
    \newcommand{\imwidth}{0.165\textwidth}
        \setlength{\tabcolsep}{0pt}
        \begin{tabular}{c@{\hskip 2pt}ccc}
        \toprule
        Original & AquaLoRA & Stable Signature & Ours (Object) \\
        \midrule

        \multicolumn{4}{c}{\textit{Prompt: A toy car in front of a \textcolor{red}{teddy bear}.}} \vspace{1mm} \\
        
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/txt2img/00_nw.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_w.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_obj.png} \\

         &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00_diff.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ss/00_diff.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_diff.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_diff.png} \\
        \midrule
        % \rule{0pt}{6ex}%

        \multicolumn{4}{c}{\textit{Prompt: A toy car in front of a \textcolor{red}{teddy bear}.}} \vspace{1mm} \\
        
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/txt2img/01_nw.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/01.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/01.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_w.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/01_diff.png} \\

         &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/01_diff.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ss/01_diff.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_diff.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/01_diff.png} \\
        \midrule

        \multicolumn{4}{c}{\textit{Prompt: A toy car in front of a \textcolor{red}{teddy bear}.}} \vspace{1mm} \\
        
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/txt2img/02_nw.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/02.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/02.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_w.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/02_obj.png} \\

         &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/02_diff.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ss/02_diff.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_diff.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/02_diff.png} \\
        \midrule

        \multicolumn{4}{c}{\textit{Prompt: A toy car in front of a \textcolor{red}{teddy bear}.}} \vspace{1mm} \\
        
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/txt2img/03_nw.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/03.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/03.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_w.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/03_obj.png} \\

         &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/03_diff.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ss/03_diff.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_diff.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/03_diff.png} \\
        \midrule

        \multicolumn{4}{c}{\textit{Prompt: A toy car in front of a \textcolor{red}{teddy bear}.}} \vspace{1mm} \\
        
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/txt2img/00_nw.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_w.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_obj.png} \\

         &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00_diff.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ss/00_diff.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_diff.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_diff.png} \\
        \midrule

        \multicolumn{4}{c}{\textit{Prompt: A toy car in front of a \textcolor{red}{teddy bear}.}} \vspace{1mm} \\
        
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/txt2img/00_nw.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_w.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_obj.png} \\

         &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00_diff.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ss/00_diff.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_diff.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_diff.png} \\
        \midrule

        \multicolumn{4}{c}{\textit{Prompt: A toy car in front of a \textcolor{red}{teddy bear}.}} \vspace{1mm} \\
        
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/txt2img/00_nw.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_w.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_obj.png} \\

         &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00_diff.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ss/00_diff.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_diff.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_diff.png} \\
        \midrule

        \multicolumn{4}{c}{\textit{Prompt: A toy car in front of a \textcolor{red}{teddy bear}.}} \vspace{1mm} \\
        
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/txt2img/00_nw.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_w.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_obj.png} \\

         &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00_diff.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ss/00_diff.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_diff.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_diff.png} \\
        \midrule

        \multicolumn{4}{c}{\textit{Prompt: A toy car in front of a \textcolor{red}{teddy bear}.}} \vspace{1mm} \\
        
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/txt2img/00_nw.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_w.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_obj.png} \\

         &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00_diff.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ss/00_diff.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_diff.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_diff.png} \\
        \midrule

        \multicolumn{4}{c}{\textit{Prompt: A toy car in front of a \textcolor{red}{teddy bear}.}} \vspace{1mm} \\
        
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/txt2img/00_nw.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_w.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_obj.png} \\

         &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00_diff.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ss/00_diff.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_diff.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_diff.png} \\
        \midrule

        \multicolumn{4}{c}{\textit{Prompt: A toy car in front of a \textcolor{red}{teddy bear}.}} \vspace{1mm} \\
        
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/txt2img/00_nw.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_w.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_obj.png} \\

         &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00_diff.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ss/00_diff.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_diff.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_diff.png} \\
        \midrule

        \multicolumn{4}{c}{\textit{Prompt: A toy car in front of a \textcolor{red}{teddy bear}.}} \vspace{1mm} \\
        
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/txt2img/00_nw.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_w.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_obj.png} \\

         &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/aqualora/00_diff.png} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ss/00_diff.png} &
        % \includegraphics[width=\imwidth]{sec/figures/supp/watermark/ssl/00_diff.jpg} &
        \includegraphics[width=\imwidth]{sec/figures/supp/qual_baselines/ours/00_diff.png} \\
        \midrule
    \\
    \end{tabular}
\caption{\label{fig:supp-watermark} Qualitative results for different watermarking methods on generated images at resolution $512$.}
\end{figure}

==> sec/tables/heatmap_breakdown.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{c}
        \toprule
        % \textbf{Heatmap breakdown} \\
        % \midrule
        \includegraphics[width=\linewidth]{sec/figures/heatmap-bk-1.png} \\ 
        % \midrule
        % \includegraphics[width=\linewidth]{sec/figures/heatmap-bk-2.png} \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Multiple Object watermarking heatmap breakdown.} \emph{Given a text prompt $\mathcal{P}$ with multiple tokens $\{\mathcal{P}_i, \mathcal{P}_j, ... \}$} selected for watermarking, we utilize attention maps of these tokens to simultaneously watermark multiple objects within the image. We present multiple objects watermarked within the generated image (first column), followed by heatmap visualization of all watermarked objects (second column), and heatmap for individual objects within the first heatmap (second column).}
    \label{tab:heatmap-breakdown}
    \vspace{-0.2in}
\end{table}

% This should be a figure


==> sec/tables/suppl_crop_table.tex <==
\begin{table}[ht]
    \centering
    \footnotesize
    
    \resizebox{\linewidth}{!}{
    \setlength{\tabcolsep}{4pt}
        \begin{tabular}{ c c c c c c c c}
        \toprule
       % & \multirow{2}{*}{Denoising timesteps}          & \multirow{2}{*}{PSNR} & \multirow{2}{*}{Bit Acc.} & \multicolumn{3}{c}{Bit Acc. Attack} \\ 

    % &                                         &                           &           & None & Crop (0.1) & Resize (0.3) \\ \midrule
\multirow{7}{*}{} 
           & \emph{\underline{Single object}} & & \emph{\underline{Bit Accuracy}} & \\ \vspace{1mm}
            &  & None & Rotate & Crop \\ 
           &     Segment + white bg           & $0.99$  & $0.97$ & $0.86$ \\ 
           &     Segment + style bg     & $0.93$  & $0.90$ & $0.83$ \\ 
           &     Crop object (0.8 $\times$ size)     & $0.89$  & $0.88$ & $0.82$ \\
           &     Crop object (0.5 $\times$ size)     & $0.89$  & $0.85$ & $0.78$ \\
           &     Crop object (0.4 $\times$ size)     & $0.76$  & $0.70$ & $0.68$ \\ \cmidrule{2-5}

           & \emph{\underline{Multiple objects}} & & \emph{\underline{Bit Accuracy}} & \\ \vspace{1mm}
            &  & None (Avg.) & Rotate (Avg.) & Crop (Avg.) \\
           &     1 object    & $0.99$  & $0.97$ & $0.86$ \\ 
           &     2 objects (no overlap)    & $0.94$&  $0.93$ & $0.85$ \\ 
           &     3 objects (no overlap)    & $0.90$&  $0.89$ & $0.83$ \\ 
           &     2 objects (overlap $\geq 40\%$)     & $0.79$  & $0.76$ & $0.70$ \\
        \bottomrule
    \end{tabular}}
    \caption{
        \textbf{Object-level watermarking robustness performance with attacks.} \emph{We evaluate the performance of our method to perform object-level watermarking in the presence of attacks. We clearly see that our method achieve robust watermarking performance on rotate and crop attacks for different crops performed within watermarked object. We present our results while watermarking single and upto three objects.} 
        \vspace*{-0.2cm}
    }\label{tab:obj_quantitative}
     
\end{table}

==> sec/tables/table2_noise_timesteps.tex <==
\begin{table}
    \centering
    \footnotesize
    
    \resizebox{\linewidth}{!}{
    \setlength{\tabcolsep}{4pt}
        \begin{tabular}{ c c c c c c c c}
        \toprule
       & \multirow{2}{*}{Timesteps}          & \multirow{2}{*}{PSNR} & \multirow{2}{*}{Bit Acc.} & \multicolumn{3}{c}{Bit Acc. Attack} \\ 

    &                                         &                           &           & Crop (0.5) & Rotate (25) & Resize (0.3) \\ \midrule
\multirow{7}{*}{} 
           & \emph{\underline{Multi-Step}} \vspace{1.5mm} \\
           &     $5$ to $0$              & $36.92$  & $0.97$ & $0.924$ & $0.585$ & $0.93$ \\ 
           &         $8$ to $0$              & $34.85$ & $0.99$ & $0.93$ & $0.585$ & $0.94$ \\ \cmidrule{2-7}

           
           & \emph{\underline{Single-Step}} \vspace{1.5mm} \\
           &    $5$ & $34.76$  & $0.94$ & $0.92$ & $0.58$ & $0.89$ \\
           &   $10$ & $33.54$  & $0.97$ & $0.91$ & $0.58$ & $0.90$ \\
           &   $100$ & $31.31$  & $0.99$ & $0.93$ & $0.58$ & $0.93$ \\
           &   $400$ & $26.87$ & $0.99$ & $0.93$ & $0.585$ & $0.93$ \\
           &   $500$ & $21.42$  & $0.96$ & $0.89$ & $0.5$ & $0.86$ \\
           &   $700$ & $14.83$   & $0.95$ & $0.88$ & $0.58$ & $0.86$ \\
           &   $900$ & $10.47$  & $0.93$ & $0.80$ & $0.5$ & $0.78$ \\

            
        \bottomrule
    \end{tabular}}
    \vspace{-3mm}
    \caption{\textbf{Optimal sub-range of noise timesteps for invisible watermarking.} \emph{We present our quantitative results for our study to find the optimal sub-range of denoising timesteps $[ \tau^* \text{ to } 0]$ for invisible watermarking. Invisible watermarking refers to high PSNR values when compared to non-watermarked images. From the table, we see that when the noise timesteps are closer to LDM decoder we achieve high invisibility for watermarking along with robust watermarking ability. From our study, we choose the optimal timestep to introduce watermarking during denoising timesteps to be $8$. {\color{red} Make this into a plot?}}
        \vspace*{-0.2cm}
    } \label{tab:noise-steps}
    % \vspace{-3mm}
\end{table}

==> sec/tables/table3_plug_and_play.tex <==
% \begin{table}
%     \centering  
%     \setlength{\tabcolsep}{4pt}
%     \scalebox{0.6}{ 
%         \begin{tabular}{ c l c c c c c c}
%         \toprule
%        & \multirow{2}{*}{}          & \multirow{2}{*}{PSNR} & \multirow{2}{*}{Bit Acc.} & \multicolumn{3}{c}{Bit Acc. Attack} \\ 

%     &                                         &                           &           & Crop (0.5) & Rotate (25) & Resize (0.3) \\ \midrule
    
%     \multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Ours}}}  % Label "Ours" vertically spanning 8 rows
%            & \underline{\textbf{Plug-In ${\mathcal{W}_*} on SD v1.5$} \vspace{1mm} \\
           
%            & lambdalabs/sd-naruto-diffusers  & $35.85$  & $0.99$ & $0.92$ & $0.92$ & $0.93$ \\ \vspace{2mm}

%            & lambdalabs/sd-pokemon-diffusers                       & $34.27$  & $0.99$ & $0.92$ & $0.92$ & $0.93$ \\ 

           
%            & \underline{\textbf{Plug-In ${\mathcal{W}_*} on SD v2.1$} \vspace{1mm} \\

%            & lavaman131/cartoonify  & $36.94$  & $0.99$ & $0.92$ & $0.92$ & $0.93$ \\ 

           
%            & Norod78/sd2-cartoon-blip & $33.94$  & $0.98$ & $0.92$ & $0.92$ & $0.91$ \\  \cmidrule{2-7}
           
%            \multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Stable Sig.}}}  % Label "Ours" vertically spanning 8 rows
%            & \emph{\underline{\textcolor{blue}{Decoder} trained on SD v1.5}}
%            \vspace{1mm} \\
           
%            & lambdalabs/sd-naruto-diffusers & $24.83$  & $0.99$ & $0.91$ & $0.87$ & $0.90$\\ \vspace{2mm}

%            & lambdalabs/sd-pokemon-diffusers  & $23.83$  & $0.99$ & $0.91$ & $0.87$ & $0.90$ \\
           
%            & \emph{\underline{\textcolor{blue}{Decoder} trained on SD v2.1}}
%            \vspace{1mm}\\
           
%            & lavaman131/cartoonify  & $23.88$  & $0.99$ & $0.91$ & $0.88$ & $0.90$ \\ 

           
%            & Norod78/sd2-cartoon-blip                       & $22.74$  & $0.99$ & $0.90$ & $0.86$ & $0.91$ \\
        
%         \bottomrule
%     \end{tabular}}
%     \caption{\textbf{Plug and Play performance on different LDM pipelines.} \emph{We evaluate the performance of our method to plug into various LDM pipelines. We see that loading the token emeddings of $\mathcal{W}_*$ for watermarking into different pipelines preserves both invisibility and robustness for watermarking until attacks.}
        
%         % \vspace*{-0.2cm}
%     }\label{tab:plug-and-play-table}
     
% \end{table}
